CFO: Conditional Focused Neural Question Answering with Large-scale Knowledge Bases

How can we enable computers to automatically answer questions like "Who created the character Harry Potter"? Carefully built knowledge bases provide rich sources of facts. However, it remains a challenge to answer factoid questions raised in natural language due to numerous expressions of one question. In particular, we focus on the most common questions --- ones that can be answered with a single fact in the knowledge base. We propose CFO, a Conditional Focused neural-network-based approach to answering factoid questions with knowledge bases. Our approach first zooms in a question to find more probable candidate subject mentions, and infers the final answers with a unified conditional probabilistic framework. Powered by deep recurrent neural networks and neural embeddings, our proposed CFO achieves an accuracy of 75.7% on a dataset of 108k questions - the largest public one to date. It outperforms the current state of the art by an absolute margin of 11.8%.

==> 032rnn.tex <==
Lies in the foundation of our method is a class of recurrent neural networks for sequence modeling.
Bidirectional RNNs \cite{schuster1997bidirectional,schuster1999supervised,baldi1999exploiting} are modified recurrent neural networks with two layers. 
For each input sequence, it learns two sequences of hidden states, a forward one and a backward one. 
Both layers are then connected to an output layer.
%As a benefit, Bidirectional RNNs are able to capture complete past and future context information, usually leading to a better prediction. 
To exploit long-range dependencies among sequences, 
earlier long-short term memory units (LSTM)~\cite{hochreiter1997long} and recent gated recurrent units (GRU) \cite{cho2014learning} have been proposed.
With trainable gates and constant error carousel (CEC), LSTM and GRU suffer less from the vanishing gradient problem \cite{bengio1994learning} 
and are able to learn long-term dependencies. 
%Compared to LSTM, GRU is able to achieve similar performance with simpler design and fewer parameters \cite{chung2014empirical,greff2015lstm,jozefowicz2015empirical}. 
%Finally, as the depth has been shown to be crucial to the success of neural networks theoretically and empirically, adding more layers to RNNs, which take the output of previous layers as input, can improve the performance of RNNs. 
Among many possible ways of constructing deep RNNs \cite{pascanu2013construct}, a widely used convention is simply stacking several layers. 
As shown in the following section, our proposed \name combines many ideas in these basic models. 

==> 053adagrad_momentum.tex <==
As the default optimization algorithm for deep neural networks, SGD has been successfully applied to different problems \cite{krizhevsky2012imagenet,sutskever2014sequence,graves2013speech}. 
However, to make good use of it, both the initial learning rate and the annealing schedule have to be tuned manually and carefully.

In comparison, AdaGrad, a SGD variant proposed by \cite{duchi2011adaptive}, has the advantage of self-adjusting (diminishing) the learning rate based on former gradients. 
Hence, we only need to tune the global learning rate of AdaGrad, which is much easier in practice. Moreover, AdaGrad adjusts the learning rate element-wise based on the geometry of the parameter space and thus enables the model to pay special attention to less-frequent (rare) features. So, when substituting SGD with AdaGrad, both the subject labeling model and the relation ranking model can achieve better and more consistent performance.
%\footnote{In our experiments, performance differences between several runs are within 0.5\%.} 

Although AdaGrad is very powerful, it continuously decreases the learning rate based on the magnitude of previous gradients. As a result, the faster the model learns, the faster the learning rate decreases. Hence, the training slows down quickly. To overcome this weakness, we propose to combine AdaGrad with Momentum, which may enable the AdaGrad to step further in the right direction accumulatively. During each parameter update, we first accumulate the velocity using the adjusted gradient 
\vspace{-0.5em}\begin{equation}
v_t = \rho_t v_{t-1} - \frac{\eta}{\sqrt{\sum_{i=1}^{t} g_i^2}}g_t \label{eq:accumulate_momentum}
\vspace{-0.5em}\end{equation}
where $g_t, v_t, \rho_t$ are the gradient, velocity, and momentum rate at time step $t$, respectively, and all math operations here are element-wise. Then, we use the accumulated velocity to perform the update
\vspace{-0.5em}\begin{equation}
\theta_t = \theta_{t-1} + v_t \label{eq:perform_update}
\vspace{-0.5em}\end{equation}
where $\theta_t$ is the parameter at time step $t$. %By adding momentum, we can step further in the right direction accumulatively. Also, since earlier updates are much larger in magnitude for AdaGrad, using momentum can partially keep these larger influences for future updates, leading to relatively faster learning at later stage.

Empirically, for the subject labeling model, combining AdaGrad with Momentum achieves the same performance in a much shorter time, allowing us to use larger dropout rate (see Section \ref{sec:dropout}). 
However, for relation ranking, directly adding momentum caused the loss to oscillate dramatically in the beginning of the training. 
Consequently, the training loss goes down very slowly, hurting the performance. 
We conjecture this is because the velocity term in early-stage hasn't accumulated enough gradients to be stable but has a large magnitude that can disrupt the direction of gradients. 
As a remedy, we propose to use momentum schedule, which disables the momentum in the beginning, and starts to increase the momentum gradually after a few epochs or when the training loss reaches a certain level. 
Intuitively, we want to avoid the noisy momentum in the early stage until it has accumulated enough gradients and become more helpful. In this work, we refer to this strategy as AdaGrad with momentum schedule.

Using AdaGrad with momentum schedule, we achieve a much lower training loss for the relation ranking model using the same training time, leading to 3.0\%+ performance improvement.

==> 060implementation.tex <==
In this section, we present some implementation details. 

==> 061database.tex <==

\paragraph{Knowledge base}
In this work, we use the latest \texttt{Freebase} \cite{google2015freebase} as the data source of our KB. The data dump contains more than 3 billion facts, where each fact is prepared in the format of N-Triples RDF. Each RDF triple has the form (subject, relation, object), as introduced in Section \ref{sec:intro}.

Instead of using all data in the \texttt{Freebase}, we consider two subsets of it for this work. 
Essentially, two principles are used to select the data. 
Firstly, the knowledge base should contain information of high practical value. 
Secondly, the data in the KB should be relevant to the dataset used in experiments (Section \ref{sec:dataset}). 
Specifically, we mainly consider entities that either have Wikipedia pages,
%\footnote{In Freebase dump, a special type of triple \textit{(subject, wikikey, wikipedia\_title)} can be used to identify such entities.}
or show up in the experiment dataset, denoted as $\mathcal{E}_{core}$. 
We believe whether being included by Wikipedia is a reasonable measure of practical usefulness, 
and we need entities in the experiment dataset to train and test our proposed system. 
For relations, we mainly consider the top 7k relations that appear most often in non-CVT triples\footnote{
Non-CVT triples are triples that don't include a compound-value-type (CVT) node as the subject or the object. 
%Since we are dealing with \sq, relations connected to CVT nodes are of no usage.
},
and also include relations in the training data, denoted as $\mathcal{R}_{core}$. 
In addition, in order to query entities by their name/alias, we include triples corresponding to such information in our KB.

Based on the principles described above, we eventually filter out two different KBs. For the first KB, we only include triples whose subject and object both belong to $\mathcal{E}_{core}$ and whose relation belongs to $\mathcal{R}_{core}$. For the second KB, we relax the requirement to include triples whose subject or object is in $\mathcal{E}_{core}$. Intuitively, the first KB only contains information between core entities, while the second one also contains information around core entities. Since the first KB is obviously smaller than the second one, we refer to them as Small-KB and Large-KB in the rest of the paper. Table \ref{tab:statistics} presents the statistics of these two KBs together with the FB-5M KB used in \cite{bordes2015large}. As we can see, the Small-KB has comparable size to the FB-5M KB, while the Large-KB is significantly larger than the other two.

\begin{table}[htb]
	\centering
	\begin{tabular}{lrrr}
		\toprule
		 & Small-KB & Large-KB & FB-5M \\ 
		\midrule
		Entities & 4.4M & 31.4M & 4.9M\\
		Relations & 7,129 & 7,129 & 7,523\\
		Triples & 25.0M & 174.5M & 22.4M\\
		\bottomrule
	\end{tabular}
	\vspace{-0.5em}
	\caption{Data statistics of the KBs used in this work and previous work.}
	\label{tab:statistics}
\end{table}

To store both KBs, we utilize the open-source version of \texttt{Virtuoso}\footnote{\url{https://github.com/openlink/virtuoso-opensource}}, a triple-store software that can directly load N-Triples RDF data into its storage. By issuing \texttt{SPARQL} queries, we can easily query different elements in the KB.

\paragraph{Question-answer linking to KB}
In order to train our system, we need a corpus of question-triple pairs, 
where the triple is the fact that can be used to answer the paired question. 

%\subsubsection{Prepare Data for Subject Labeling}
\label{sec:subject_linking_data}
To train the subject labeling model, we need the correct label of which part is describing the subject in the question. 
Based on the question-triple pairs, we can obtain this label by reverse linking. 
For each question, there is a correct subject from the corresponding triple. 
Thus, we can issue a query to the KB for the name/alias of the subject. 
Then, we try to match each name/alias with all substrings of question. 
Once a match is found, we know the substring is referring to the entity. Thus, we can obtain the correct label. 
If there are several matches, we only choose the longest substring as the correct label. 
Using this method, 95.6\% of the original training data can have a match and thus be used for training. 

%\subsubsection{Prepare Data for Relation Ranking}
\label{sec:relation_raking_data}
As described in Section \ref{sec:relation_ranking}, to train the relation ranking model, we need extra negative samples. 
For this specific task, since there is only one correct relation for a question, all other relations appearing in the training set can be used as negative samples. Specifically, from 7,129 unique relations stored in the KB, we randomly sample 6,912
%\footnote{This number is chosen to ensure the efficient computation.} 
unique negative samples for each pair of question and positive relation. Because the two relations \textit{type.object.type} and \textit{common.topic.notable\_types} are connected to nearly all entities in the KB, the system tends to bias towards them mistakenly when the correct relation appears rarely in the training data. 
Thus, we make sure that these two relations are always sampled if they are not the correct one.



==> 063preprocess.tex <==
In this work, we take use of \texttt{Torch}\footnote{\url{http://torch.ch/}} to implement all our models. 

==> 065subject_query.tex <==
%Describe how to use the subject labeling results to query candidate subjects

==> 077error_analysis.tex <==
Finally, we present a series of error analysis to explain why our system fails in different cases. Figure \ref{fig:confusion_matrix} shows the confusion matrices.
%\footnote{The numbers presented here are essentially the same as those in Figure \ref{fig:pipeline_performance} but in another form for easier understanding.}

\begin{figure}[h]
	\centering
	\includegraphics[scale=0.39]{FIG/confusion_matrix.pdf}
	\caption{Confusion matrices showing error statistics of our system in percentage under different KBs.}
	\label{fig:confusion_matrix}
\end{figure}

\textbf{Correct Relation \& Incorrect Subject} As shown in the figure, this type of error is the biggest source of the error. 
By manually reviewing 100 randomly sampled errors of this type, we found that none of these errors is really erratic. 
Firstly, 12\% the predicted subjects and the annotated subjects are actually referring to the same entity in reality. 
Secondly, 1\% of questions have constraints on the subject, which are not really \sq. 
More surprisingly, the remaining 87\% all fall into the case that there are multiple entities with not only the same name/alias but also the same type in KB. 
Therefore, it's essentially indistinguishable even for human beings. 
This result suggests that once the relation is correctly ranked, our heuristic disambiguation method is actually pretty good. 
%More importantly, it suggests that such ambiguous questions can only be answered either when extra constraint is explicitly stated in the question, or when further human-computer interaction is allowed to provide more information. 

\textbf{Incorrect Relation \& Correct Subject} This type of error basically means that the model may choose the right subject for the wrong reason (relation). 
Again, we manually checked 70 error cases, and found these errors can be divided into 3 categories. 
Firstly, only 36\% of them can be confidently classified as ranking errors. 
For the rest, they either belong to annotation errors (7\%) or have arguable annotations (57\%). 
A typical example of arguable annotation is the decision between \textit{music.release.track\_list} and \textit{music.release.track} when asking about \textit{``what is a track of the album [name]''}. 
From human's perspective, both relations are  correct, but only one of them was labeled as correct in annotation. 
Actually, we find that such similar relations are used almost interchangeably in annotation.

\textbf{Incorrect Relation \& Incorrect Subject} Even when the predicted relation and subject are both incorrect, it doesn't necessarily mean that the model truly makes a mistake. 
Out of 80 randomly sampled errors we manually reviewed, most errors (60\%) fall into the case that although the annotated subject and the predicted subject (with the same name/alias) have different types, they can both fit into the context of question but imply different relations. 
For example, in the question \textit{``What genre is the Scar?''}, \textit{``the Scar''} can refer to a book or a film, implying the relation \textit{book.book.genre} or \textit{film.film.genre} respectively. 
Besides, there are about 13\% of annotation errors, leaving only 27\% of real mistakes. 
Note that this specific ambiguity only occurred in the multi-subject case, which explains the last observation in Section \ref{sec:results}.
